Investigating methods to improve photovoltaic thermal models at second-to-minute timescales

This paper presents a range of methods to improve the accuracy of equation-based thermal models of PV modules at second-to-minute timescales. We present an RC-equivalent conceptual model for PV modules, where wind effects are captured. We show how the thermal time constant $\tau$ of PV modules can be determined from measured data, and subsequently used to make static thermal models dynamic by applying the Exponential Weighted Mean (EWM) approach to irradiance and wind signals. On average, $\tau$ is $6.3 \pm 1~$min for fixed-mount PV systems. Based on this conceptual model, the Filter- EWM - Mean Bias Error correction (FEM) methodology is developed. We propose two thermal models, WM1 and WM2, and compare these against the models of Ross, Sandia, and Faiman on twenty-four datasets of fifteen sites, with time resolutions ranging from 1$~$s to 1$~$h, the majority of these at 1$~$min resolution. The FEM methodology is shown to reduce model errors (RMSE and MAE) on average for all sites and models versus the standard steady-state equivalent by -1.1$~$K and -0.75$~$K respectively.

==> KUL_NIST_RMSE_MAE_vals_leq_1T_std_vs_FEM_table.tex <==
\begin {tabular}{XYZZZcZZ}%
\toprule \multicolumn {1}{c}{Org}&\multicolumn {1}{c}{KPI}&\multicolumn {1}{c}{WM1}&\multicolumn {1}{c}{WM2}&\multicolumn {1}{c}{Ross}&\multicolumn {1}{c}{Sandia}&\multicolumn {1}{c}{Faiman}&\multicolumn {1}{c}{Average}\\\hline %
KUL&RMSE std [K]&3.26&3.73&3.02&2.66&2.86&3.11\\%
KUL&RMSE FEM [K]&1.4&1.52&2.12&2.08&1.56&1.74\\%
KUL&$\Delta $RMSE [K]&-1.86&-2.21&-0.9&-0.58&-1.31&-1.37\\%
KUL&$\Delta $RMSE [\%]&-57.1&-59.2&-30.0&-21.6&-45.7&-44.2\\\hline %
NIST&RMSE std [K]&3.48&3.95&3.71&3.33&3.36&3.56\\%
NIST&RMSE FEM [K]&1.87&1.83&2.85&2.38&2.19&2.22\\%
NIST&$\Delta $RMSE [K]&-1.6&-2.12&-0.86&-0.95&-1.16&-1.34\\%
NIST&$\Delta $RMSE [\%]&-46.2&-53.7&-23.2&-28.5&-34.7&-37.6\\\hline %
KUL&MAE std [K]&2.34&2.71&2.13&1.81&1.99&2.19\\%
KUL&MAE FEM [K]&1.11&1.26&1.54&1.5&1.13&1.31\\%
KUL&$\Delta $MAE [K]&-1.22&-1.45&-0.59&-0.31&-0.86&-0.89\\%
KUL&$\Delta $MAE [\%]&-52.5&-53.5&-27.9&-16.9&-43.2&-40.4\\\hline %
NIST&MAE std [K]&2.5&2.92&2.67&2.31&2.33&2.55\\%
NIST&MAE FEM [K]&1.4&1.44&2.11&1.78&1.62&1.67\\%
NIST&$\Delta $MAE [K]&-1.1&-1.49&-0.56&-0.53&-0.71&-0.88\\%
NIST&$\Delta $MAE [\%]&-43.8&-50.9&-21.0&-22.8&-30.5&-34.4\\\bottomrule %
\end {tabular}%


==> MAE_FEM_std_all_models_all_sites_table.tex <==

\newcolumntype{P}{>{\centering\arraybackslash}p{0.12\linewidth}}
\newcolumntype{Q}{>{\centering\arraybackslash}p{0.055\linewidth}}

\begin {tabular}{Qc|ccccc|ccccc}%
\toprule Org & Site & \multicolumn {5}{c}{FEM}&\multicolumn {5}{c}{standard}\\%
&&WM1&WM2&Ross&Sand&Faim&WM1&WM2&Ross&Sand&Faim\\\hline %
KUL&B roof 1s&1.12&1.29&1.54&1.51&1.12&2.49&2.87&2.17&1.88&2.14\\%
KUL&B roof 1min&1.1&1.23&1.53&1.5&1.14&2.18&2.55&2.09&1.74&1.84\\%
KUL&B roof 5min&1.2&1.37&1.55&1.52&1.18&2.03&2.48&1.93&1.57&1.6\\%
KUL&B roof 15min&1.26&1.26&1.55&1.49&1.42&1.35&1.38&1.98&1.41&1.4\\%
KUL&B roof 1h&1.12&1.22&1.46&1.37&1.28&1.18&1.23&1.99&1.24&1.2\\%
KUL&APV HAX front&1.35&1.37&1.36&1.36&1.36&1.31&1.28&1.25&1.24&1.27\\%
NIST&Ground RTD 4 10s&1.4&1.43&2.11&1.78&1.61&2.6&3.01&2.7&2.37&2.42\\%
NIST&Ground RTD 4 1min&1.41&1.44&2.11&1.78&1.63&2.4&2.84&2.64&2.24&2.24\\%
NIST&Ground RTD 4 5min&1.47&1.62&2.14&1.83&1.59&2.38&3.09&2.49&2.05&2.02\\%
NIST&Ground RTD 4 15min&1.74&1.67&2.09&1.8&1.97&1.83&1.8&2.4&1.88&2.02\\%
NIST&Ground RTD 4 1h&1.71&1.63&2.0&1.73&1.93&1.71&1.64&2.3&1.72&1.91\\%
NIST&Ground RTD 8 10s&1.45&1.59&2.19&1.91&1.56&3.15&3.73&2.87&2.54&2.73\\%
NIST&Canopy E RTD 4 10s&1.55&2.18&2.03&1.64&1.29&3.61&4.64&2.63&2.38&2.83\\%
NIST&Canopy W 10s&1.32&1.58&1.99&1.8&1.39&3.2&3.89&2.83&2.6&2.78\\%
DOE&c10hov6&1.99&2.21&2.67&2.04&2.32&2.52&2.8&3.33&2.54&2.78\\%
DOE&t3pg1sv&2.09&2.35&2.69&2.22&2.38&2.58&2.87&3.44&2.65&2.8\\%
DOE&wca0c5m&1.84&1.82&2.2&1.94&1.82&2.98&3.05&3.62&3.05&3.04\\%
DOE&z0aygry&1.49&1.47&1.99&1.76&1.49&3.03&3.15&3.9&3.01&3.06\\%
DOE&lwcb907&1.45&1.41&2.11&2.53&1.77&3.06&3.25&3.3&2.81&2.82\\%
DOE&luemkoy&1.21&1.24&1.95&1.83&1.36&2.37&2.52&2.53&2.18&2.19\\%
NREL&Sanyo&1.48&1.67&2.17&1.61&1.33&2.81&3.17&2.41&2.09&2.28\\%
U. H.&System 1&1.54&1.87&1.81&2.21&1.54&2.53&2.44&2.5&2.58&2.49\\%
U. H.&System 2A&1.13&1.72&1.95&1.09&1.2&2.07&2.73&2.64&2.0&2.15\\%
U. H.&System 2B&1.73&1.52&1.69&1.68&1.77&2.31&2.25&2.26&2.25&2.29\\%
\hline Avg&all&1.46&1.59&1.95&1.75&1.56&2.4&2.69&2.59&2.17&2.26\\\bottomrule %
\end {tabular}%


==> MBE_FEM_std_all_models_all_sites_table.tex <==
\newcolumntype{P}{>{\centering\arraybackslash}p{0.12\linewidth}}
\newcolumntype{Q}{>{\centering\arraybackslash}p{0.055\linewidth}}

\begin {tabular}{Qc|ccccc|ccccc}%
\toprule Org & Site & \multicolumn {5}{c}{FEM}&\multicolumn {5}{c}{standard}\\%
&&WM1&WM2&Ross&Sand&Faim&WM1&WM2&Ross&Sand&Faim\\\hline %
KUL&B roof 1s&-0.01&0.02&0.25&0.09&-0.02&-1.71&-2.21&-1.08&0.01&-0.96\\%
KUL&B roof 1min&-0.01&0.01&0.24&0.08&-0.02&-1.53&-2.02&-1.08&0.04&-0.78\\%
KUL&B roof 5min&-0.02&0.0&0.24&0.09&-0.02&-1.64&-2.21&-1.08&0.05&-0.81\\%
KUL&B roof 15min&0.0&-0.03&0.24&0.08&0.01&-0.46&-0.44&-1.51&0.0&-0.08\\%
KUL&B roof 1h&0.01&-0.06&0.24&0.06&0.01&-0.65&-0.3&-1.75&-0.07&-0.21\\%
KUL&APV HAX front&-0.09&-0.09&-0.06&-0.07&-0.09&-0.3&-0.23&-0.0&0.04&-0.2\\%
NIST&Ground RTD 4 10s&0.17&0.16&0.08&0.15&0.17&-1.27&-2.02&-0.7&0.16&-0.4\\%
NIST&Ground RTD 4 1min&0.17&0.17&0.08&0.15&0.17&-1.21&-1.98&-0.7&0.17&-0.31\\%
NIST&Ground RTD 4 5min&0.17&0.17&0.09&0.15&0.17&-1.67&-2.64&-0.7&0.19&-0.58\\%
NIST&Ground RTD 4 15min&0.16&0.17&0.09&0.15&0.15&0.05&-0.28&-1.14&0.16&0.51\\%
NIST&Ground RTD 4 1h&0.15&0.17&0.08&0.15&0.14&0.06&-0.29&-1.37&0.06&0.49\\%
NIST&Ground RTD 8 10s&0.23&0.22&0.14&0.2&0.23&-2.1&-2.95&-0.91&0.12&-1.09\\%
NIST&Canopy E RTD 4 10s&0.02&-0.01&-0.11&-0.0&0.02&-2.92&-4.13&-0.74&0.18&-1.59\\%
NIST&Canopy W 10s&0.07&0.06&-0.03&0.07&0.08&-2.3&-3.22&-1.12&0.06&-1.31\\%
DOE&c10hov6&0.11&0.18&-0.18&0.11&0.09&0.35&0.96&-1.87&0.43&0.94\\%
DOE&t3pg1sv&0.15&0.22&-0.15&0.13&0.13&0.21&0.85&-2.0&0.44&0.76\\%
DOE&wca0c5m&-0.01&-0.01&0.01&-0.0&-0.01&0.96&1.14&2.95&0.27&1.16\\%
DOE&z0aygry&0.05&0.05&0.07&0.05&0.05&1.88&2.13&3.48&0.29&1.98\\%
DOE&lwcb907&0.04&0.03&0.35&0.2&0.04&-2.16&-2.51&-2.0&0.1&-1.37\\%
DOE&luemkoy&-0.05&-0.06&0.25&0.11&-0.04&-1.43&-1.73&-0.9&0.19&-0.76\\%
NREL&Sanyo&0.05&0.04&0.09&0.05&0.06&-1.86&-2.37&0.41&0.27&-0.88\\%
U. H.&System 1&0.84&0.83&0.8&0.7&0.81&-1.52&-0.47&-1.5&0.62&-1.45\\%
U. H.&System 2A&0.15&0.12&0.07&0.21&0.08&0.82&1.85&1.46&0.24&1.05\\%
U. H.&System 2B&0.33&0.3&0.2&0.28&0.32&0.25&-0.28&0.17&0.13&0.26\\%
\hline Avg&all&0.11&0.11&0.13&0.13&0.11&-0.84&-1.06&-0.57&0.17&-0.23\\\bottomrule %
\end {tabular}%


==> RMSE_FEM_std_all_models_all_sites_table.tex <==
\newcolumntype{P}{>{\centering\arraybackslash}p{0.12\linewidth}}
\newcolumntype{Q}{>{\centering\arraybackslash}p{0.055\linewidth}}

\begin {tabular}{Qc|ccccc|ccccc}%
\toprule Org & Site & \multicolumn {5}{c}{FEM}&\multicolumn {5}{c}{standard}\\%
&&WM1&WM2&Ross&Sand&Faim&WM1&WM2&Ross&Sand&Faim\\\hline %
KUL&B roof 1s&1.39&1.54&2.12&2.09&1.53&3.53&4.01&3.12&2.78&3.1\\%
KUL&B roof 1min&1.41&1.5&2.11&2.08&1.58&3.0&3.45&2.92&2.54&2.63\\%
KUL&B roof 5min&1.51&1.65&2.13&2.12&1.63&2.65&3.17&2.57&2.23&2.2\\%
KUL&B roof 15min&1.76&1.75&2.06&2.08&1.98&1.84&1.87&2.52&1.96&1.92\\%
KUL&B roof 1h&1.55&1.69&1.91&1.9&1.79&1.58&1.66&2.47&1.69&1.63\\%
KUL&APV HAX front&1.77&1.79&1.77&1.77&1.78&1.74&1.71&1.7&1.67&1.69\\%
NIST&Ground RTD 4 10s&1.86&1.82&2.85&2.38&2.18&3.62&4.09&3.77&3.43&3.48\\%
NIST&Ground RTD 4 1min&1.88&1.84&2.85&2.38&2.2&3.33&3.81&3.65&3.23&3.23\\%
NIST&Ground RTD 4 5min&1.92&2.03&2.89&2.45&2.17&3.15&3.94&3.38&2.93&2.87\\%
NIST&Ground RTD 4 15min&2.34&2.24&2.82&2.41&2.6&2.56&2.55&3.27&2.66&2.86\\%
NIST&Ground RTD 4 1h&2.27&2.16&2.69&2.29&2.53&2.37&2.33&3.14&2.43&2.68\\%
NIST&Ground RTD 8 10s&1.91&2.0&2.94&2.58&2.16&4.33&4.99&4.04&3.7&3.93\\%
NIST&Canopy E RTD 4 10s&1.98&2.68&2.68&2.15&1.72&4.85&5.99&3.69&3.43&4.01\\%
NIST&Canopy W 10s&1.7&1.98&2.59&2.34&1.84&4.33&5.09&3.94&3.72&3.93\\%
DOE&c10hov6&2.44&2.7&3.52&2.51&2.79&3.43&3.72&4.45&3.41&3.67\\%
DOE&t3pg1sv&2.6&2.9&3.51&2.75&2.91&3.5&3.81&4.54&3.53&3.69\\%
DOE&wca0c5m&2.36&2.34&2.79&2.48&2.34&4.07&4.12&4.81&4.18&4.1\\%
DOE&z0aygry&2.05&2.04&2.57&2.36&2.05&4.14&4.23&4.98&4.17&4.15\\%
DOE&lwcb907&2.13&2.05&2.98&3.25&2.47&3.97&4.19&4.21&3.67&3.68\\%
DOE&luemkoy&1.78&1.78&2.74&2.45&1.97&3.36&3.56&3.53&3.1&3.14\\%
NREL&Sanyo&2.05&2.26&3.01&2.29&1.9&3.72&4.12&3.36&2.94&3.14\\%
U. H.&System 1&2.01&2.57&2.37&2.89&2.03&3.57&3.54&3.59&3.48&3.56\\%
U. H.&System 2A&1.48&2.47&2.63&1.44&1.55&3.02&3.74&3.63&2.98&3.1\\%
U. H.&System 2B&2.26&2.1&2.33&2.25&2.3&3.24&3.18&3.2&3.18&3.21\\%
\hline Avg&all&1.93&2.08&2.62&2.32&2.08&3.29&3.62&3.52&3.04&3.15\\\bottomrule %
\end {tabular}%


==> mean_RMSE_MAE_results_differences_all_sites_all_models_table.tex <==
\newcolumntype{K}{>{\centering\arraybackslash}p{0.05\linewidth}}
\newcolumntype{L}{>{\centering\arraybackslash}p{0.20\linewidth}}
\newcolumntype{M}{>{\centering\arraybackslash}p{0.065\linewidth}}

\begin {tabular}{cKKKcMM}%
\toprule Model&WM1&WM2&Ross&Sandia&Faiman&Average\\\hline %
RMSE$_{std}$ [K]&3.29&3.62&3.52&3.04&3.15&3.32\\%
RMSE$_{FEM}$ [K]&1.93&2.08&2.62&2.32&2.08&2.21\\%
$\Delta $RMSE [K]&-1.36&-1.54&-0.9&-0.72&-1.07&-1.12\\%
$\Delta $RMSE [\%]&-41.3&-42.5&-25.6&-23.7&-34.0&-33.4\\%
$\sigma _{RMSE-std}$ [K]&0.84&1.05&0.78&0.7&0.74&0.82\\%
$\sigma _{RMSE-FEM}$ [K]&0.34&0.38&0.45&0.36&0.39&0.38\\\hline %
MAE$_{std}$ [K]&2.4&2.69&2.59&2.17&2.26&2.42\\%
MAE$_{FEM}$ [K]&1.46&1.59&1.95&1.75&1.56&1.66\\%
$\Delta $MAE [K]&-0.94&-1.1&-0.64&-0.42&-0.7&-0.76\\%
$\Delta $MAE [\%]&-39.2&-40.9&-24.7&-19.4&-31.0&-31.0\\%
$\sigma _{MAE-std}$ [K]&0.63&0.82&0.6&0.52&0.54&0.62\\%
$\sigma _{MAE-FEM}$ [K]&0.27&0.31&0.34&0.31&0.34&0.31\\\hline %
MBE$_{std}$ [K]&-0.84&-1.06&-0.57&0.17&-0.23&-0.51\\%
MBE$_{FEM}$ [K]&0.11&0.11&0.13&0.13&0.11&0.12\\%
$\Delta | \text {MBE}|$ [K]&-0.73&-0.95&-0.44&-0.04&-0.12&-0.46\\\bottomrule %
\end {tabular}%


==> r_eq_c_eq_tau_values_WM1_all_sites_table.tex <==
\newcolumntype{F}{>{\centering\arraybackslash}p{0.21\linewidth}}
\newcolumntype{G}{>{\centering\arraybackslash}p{0.0425\linewidth}}
\newcolumntype{H}{>{\centering\arraybackslash}p{0.0525\linewidth}}
\newcolumntype{I}{>{\centering\arraybackslash}p{0.0325\linewidth}}

\begin {tabular}{HFGGGGGGIIII}%
\toprule Org.&Site&$r_{eq,max}$ $\big [\frac {mK}{W/m^2}\big ]$&$r_M$ $\big [\frac {mK}{W/m^2}\big ]$&$r_{film}$ $\big [\frac {mK}{W/m^2}\big ]$&$c_{eq,max}$ $\big [\frac {kJ}{K\cdot m^2}\big ]$&$c_M$ $\big [\frac {kJ}{K\cdot m^2}\big ]$&$c_{film}$ $\big [\frac {kJ}{K\cdot m^2}\big ]$&$\tau _0$ \quad $[s]$&$\tau $ \quad $[s]$&$\Delta t$ \quad $[s]$&$f$ \quad $\big [\frac {s}{m}\big ]$\\\hline %
KUL&B roof 1s&35.4&15.3&20.1&37.7&26.9&10.8&576&410&1&11.8\\%
KUL&B roof 1min&34.8&15.3&19.5&37.4&23.8&13.6&572&364&60&15.53\\%
KUL&B roof 5min&35.4&15.6&19.8&37.5&22.6&14.9&584&352&300&13.82\\%
KUL&B roof 15min&31.2&16.3&14.9&53.7&27.8&25.9&874&453&900&10.64\\%
KUL&B roof 1h&31.4&17.0&14.4&211.8&-&-&-&-&3600&-\\\hline %
KUL&APV HAX front&12.2&5.3&6.9&102.8&16.6&86.2&545&87&60&2.74\\\hline %
NIST&Ground RTD 4 10s&31.3&14.0&17.3&36.4&23.6&12.8&510&330&10&16.16\\%
NIST&Ground RTD 4 1min&31.2&14.0&17.2&36.5&23.9&12.6&510&334&60&16.56\\%
NIST&Ground RTD 4 5min&32.7&14.0&18.7&35.5&23.7&11.8&497&332&300&14.91\\%
NIST&Ground RTD 4 15min&28.0&15.1&12.9&56.4&31.0&25.4&851&468&900&10.02\\%
NIST&Ground RTD 4 1h&28.2&15.3&12.9&235.3&-&-&-&-&3600&-\\\hline %
NIST&Ground RTD 8 10s&36.2&16.8&19.4&30.5&21.5&9.0&513&361&10&19.98\\%
NIST&Canopy E RTD 4 10s&41.6&17.2&24.4&27.1&14.0&13.1&465&241&10&12.17\\%
NIST&Canopy W 10s&38.2&18.5&19.7&27.6&16.0&11.6&511&295&10&14.57\\\hline %
DOE&c10hov6&35.0&18.5&16.5&40.7&22.3&18.4&753&412&60&16.57\\%
DOE&t3pg1sv&34.9&18.8&16.1&39.9&22.7&17.2&750&426&60&17.73\\\hline %
DOE&wca0c5m&30.7&18.6&12.1&31.5&25.5&6.0&586&474&60&33.14\\%
DOE&z0aygry&30.1&18.0&12.1&32.4&25.4&7.0&583&456&60&28.63\\\hline %
DOE&lwcb907&37.2&19.1&18.1&29.7&20.0&9.7&567&382&60&20.24\\%
DOE&luemkoy&35.8&17.7&18.1&32.1&21.6&10.5&567&381&60&20.18\\\hline %
NREL&Sanyo&32.2&16.3&15.9&40.2&25.7&14.5&655&418&60&11.17\\\hline %
U. H.&System 1&31.5&19.9&11.6&37.8&16.4&21.4&751&326&60&4.8\\%
U. H.&System 2A&32.2&16.4&15.8&32.4&28.8&3.6&532&472&60&33.76\\%
U. H.&System 2B&23.1&16.4&6.7&31.8&25.9&5.9&522&425&60&24.33\\\hline %
Average&$\Delta t<900 \: s$&32.6&16.3&16.3&37.9&22.3&15.5&577&364&-&17.44\\\bottomrule %
\end {tabular}%

